QED corrections to neutron and nuclear $\beta$-decay at order $\alpha^2$

We compute two-loop QED corrections to neutron and nuclear beta decay, including full electron mass dependence and real radiation contributions. The result for the neutron, $\delta_{R,\,\rm static}= ( 29.199 \pm 0.001 )\times 10^{-3}$, implies a factor $\sim 70 $ reduction in the uncertainty of the low-energy radiative corrections compared to previous results obtained in the large energy/small electron-mass limit, $m_e/(m_n-m_p) \to 0$. For superallowed nuclear decays we find that the $Z$-independent order $\alpha^2$ corrections range from $(0.1-0.5) \times 10^{-4}$ i.e., of roughly the expected size and comparable to current uncertainty estimates.

==> code/numerics/RV_tq_blocks.tex <==
% RV_tq_blocks.tex -- the functions F_a, F_b, F_c, F_d of the T_q term (App. B), generated from analytic/tq_F.expr.json.
% l_X = \ln|X| with X in {\zeta, R, 1+R, R+\zeta^2, 1+R\zeta^2, \zeta^2-1, \zeta^2+1, 1-R};
% g_R = \ln(R/(1+R)^2), h_R = 2\ln|(1-R)/(1+R)|; Li_2 real part; S(A,B) = \int_0^1 dt/t \ln|1-At|\ln|1-Bt|.
\begin{align*}F_a(\zeta,R)&=\Bigl(- 2 P_{q}\Bigr)\mathrm{Li}_2\!\left(- \frac{1}{\left(\zeta - 1\right) \left(\zeta + 1\right)}\right)\\&\quad+\Bigl(\frac{2 P_{q} \zeta^{2}}{\left(\zeta - 1\right) \left(\zeta + 1\right)}\Bigr)\mathrm{Li}_2\!\left(- \frac{R \left(\zeta - 1\right) \left(\zeta + 1\right)}{R + \zeta^{2}}\right)\\&\quad+\Bigl(\frac{2 P_{q} \zeta^{2}}{\left(\zeta - 1\right) \left(\zeta + 1\right)}\Bigr)\mathrm{Li}_2\!\left(- \frac{\left(\zeta - 1\right) \left(\zeta + 1\right)}{R \zeta^{2} + 1}\right)\\&\quad+\Bigl(\frac{2 P_{q} \left(\zeta^{2} + 1\right)}{\left(\zeta - 1\right) \left(\zeta + 1\right)}\Bigr)\mathrm{Li}_2\!\left(\frac{1}{R + 1}\right)\\&\quad+\Bigl(- \frac{2 P_{q} \left(R + \zeta^{2}\right)}{\left(R + 1\right) \left(\zeta - 1\right) \left(\zeta + 1\right)}\Bigr)\mathrm{Li}_2\!\left(\frac{1}{R \zeta^{2} + 1}\right)\\&\quad+\Bigl(\frac{2 P_{q} R}{R + 1}\Bigr)\mathrm{Li}_2\!\left(\frac{\zeta^{2} \left(R + 1\right)}{R + \zeta^{2}}\right)\\&\quad+\Bigl(\frac{2 P_{q}}{R + 1}\Bigr)\mathrm{Li}_2\!\left(\frac{\zeta^{2} \left(R + 1\right)}{R \zeta^{2} + 1}\right)\\&\quad+\Bigl(\frac{2 P_{q}}{\left(\zeta - 1\right) \left(\zeta + 1\right)}\Bigr)\mathrm{Li}_2\!\left(\frac{R \left(\zeta - 1\right) \left(\zeta + 1\right)}{R \zeta^{2} + 1}\right)\\&\quad+\Bigl(- \frac{2 P_{q} \left(R + \zeta^{2}\right)}{\left(R + 1\right) \left(\zeta - 1\right) \left(\zeta + 1\right)}\Bigr)\mathrm{Li}_2\!\left(\frac{R \zeta^{2}}{R \zeta^{2} + 1}\right)\\&\quad+\Bigl(\frac{2 P_{q} \left(\zeta^{2} + 1\right)}{\left(\zeta - 1\right) \left(\zeta + 1\right)}\Bigr)\mathrm{Li}_2\!\left(\frac{R}{R + 1}\right)\\&\quad+\Bigl(- \frac{2 P_{q}}{R + 1}\Bigr)\mathrm{Li}_2\!\left(\frac{R + 1}{R + \zeta^{2}}\right)\\&\quad+\Bigl(- \frac{2 P_{q} \left(R \zeta^{2} + 1\right)}{\left(R + 1\right) \left(\zeta - 1\right) \left(\zeta + 1\right)}\Bigr)\mathrm{Li}_2\!\left(\frac{R}{R + \zeta^{2}}\right)\\&\quad+\Bigl(- \frac{2 P_{q} R}{R + 1}\Bigr)\mathrm{Li}_2\!\left(\frac{R + 1}{R \zeta^{2} + 1}\right)\\&\quad+\Bigl(\frac{2 P_{q}}{\left(\zeta - 1\right) \left(\zeta + 1\right)}\Bigr)\mathrm{Li}_2\!\left(\frac{\left(\zeta - 1\right) \left(\zeta + 1\right)}{R + \zeta^{2}}\right)\\&\quad+\Bigl(- \frac{2 P_{q} \left(R \zeta^{2} + 1\right)}{\left(R + 1\right) \left(\zeta - 1\right) \left(\zeta + 1\right)}\Bigr)\mathrm{Li}_2\!\left(\frac{\zeta^{2}}{R + \zeta^{2}}\right)\\&\quad+\Bigl(2 P_{q}\Bigr)\mathrm{Li}_2\!\left(\frac{\zeta^{2}}{\left(\zeta - 1\right) \left(\zeta + 1\right)}\right)\\&\quad+\frac{1}{\left(R + 1\right) \left(\zeta - 1\right) \left(\zeta + 1\right)}\Bigl[- 4 P_{q} \ell_{1+R} - 2 P_{q} g_{R} + 2 P_{q} \ell_{R} - 4 P_{q} \ell_{R} \ell_{\zeta}\\&\qquad- 4 P_{q} R \ell_{1+R} - 4 P_{q} \zeta^{2} \ell_{1+R} - 2 P_{q} g_{R} \ell_{\zeta^2-1} - 2 P_{q} R g_{R}\\&\qquad- 2 P_{q} \zeta^{2} g_{R} - 2 P_{q} \ell_{R} \ell_{1+R\zeta^2} - 2 P_{q} \ell_{1+R\zeta^2} \ell_{\zeta^2-1} - 2 P_{q} \ell_{1+R} \ell_{R+\zeta^2}\\&\qquad- 2 P_{q} \ell_{R+\zeta^2} \ell_{\zeta^2-1} + 2 P_{q} \ell_{R} \ell_{R+\zeta^2} + 2 P_{q} \ell_{R} \ell_{\zeta^2-1} + 2 P_{q} R \ell_{R}\\&\qquad+2 P_{q} \zeta^{2} \ell_{R} + 2 P_{q} \ell_{1+R\zeta^2} \ell_{1+R} + 4 P_{q} \ell_{\zeta} \ell_{1+R\zeta^2} + 4 P_{q} \ell_{\zeta} \ell_{R+\zeta^2}\\&\qquad- 4 P_{q} R \ell_{R} \ell_{\zeta} - 4 P_{q} R \zeta^{2} \ell_{1+R} - 2 P_{q} R g_{R} \ell_{\zeta^2-1} - 2 P_{q} \zeta^{2} g_{R} \ell_{\zeta^2-1}\\&\qquad- 2 P_{q} R \zeta^{2} g_{R} - 2 P_{q} \zeta^{2} \ell_{R} \ell_{R+\zeta^2} - 2 P_{q} R \ell_{1+R\zeta^2} \ell_{1+R} - 2 P_{q} \zeta^{2} \ell_{1+R\zeta^2} \ell_{1+R}\\&\qquad- 2 P_{q} R \ell_{1+R\zeta^2} \ell_{\zeta^2-1} - 2 P_{q} \zeta^{2} \ell_{1+R\zeta^2} \ell_{\zeta^2-1} - 2 P_{q} R \ell_{R+\zeta^2} \ell_{\zeta^2-1} - 2 P_{q} \zeta^{2} \ell_{R+\zeta^2} \ell_{\zeta^2-1}\\&\qquad+2 P_{q} \zeta^{2} \ell_{R} \ell_{1+R\zeta^2} + 2 P_{q} R \ell_{R} \ell_{\zeta^2-1} + 2 P_{q} \zeta^{2} \ell_{R} \ell_{\zeta^2-1} + 2 P_{q} R \zeta^{2} \ell_{R}\\&\qquad+2 P_{q} R \ell_{1+R} \ell_{R+\zeta^2} + 2 P_{q} \zeta^{2} \ell_{1+R} \ell_{R+\zeta^2} + 4 P_{q} \zeta^{2} g_{R} \ell_{\zeta} + 4 P_{q} R \ell_{\zeta} \ell_{1+R\zeta^2}\\&\qquad+4 P_{q} R \ell_{\zeta} \ell_{R+\zeta^2} + 8 P_{q} \zeta^{2} \ell_{\zeta} \ell_{\zeta^2-1} - 2 P_{q} R \zeta^{2} g_{R} \ell_{\zeta^2-1} - 2 P_{q} R \zeta^{2} \ell_{1+R\zeta^2} \ell_{\zeta^2-1}\\&\qquad- 2 P_{q} R \zeta^{2} \ell_{1+R} \ell_{R+\zeta^2} - 2 P_{q} R \zeta^{2} \ell_{R+\zeta^2} \ell_{\zeta^2-1} + 2 P_{q} R \zeta^{2} \ell_{R} \ell_{\zeta^2-1} + 2 P_{q} R \zeta^{2} \ell_{1+R\zeta^2} \ell_{1+R}\\&\qquad+4 P_{q} R \zeta^{2} g_{R} \ell_{\zeta} + 8 P_{q} R \zeta^{2} \ell_{\zeta} \ell_{\zeta^2-1}\Bigr]\end{align*}

\begin{align*}F_b(\zeta,R)&=\Bigl(\frac{\zeta^{4} - 4 \zeta^{2} \ell_{\zeta} - 1}{8 P_{q}^{3} \zeta^{2}}\Bigr)\mathrm{Li}_2\!\left(- \frac{1}{R}\right)\\&\quad+\Bigl(\frac{\zeta^{4} - 4 \zeta^{2} \ell_{\zeta} - 1}{8 P_{q}^{3} \zeta^{2}}\Bigr)\mathrm{Li}_2\!\left(- R\right)\\&\quad+\Bigl(- \frac{\left(\zeta - 1\right) \left(\zeta + 1\right) \left(\zeta^{2} + 1\right)}{8 P_{q}^{3} \zeta^{2}}\Bigr)\mathrm{Li}_2\!\left(- \frac{R \left(\zeta - 1\right) \left(\zeta + 1\right)}{R + \zeta^{2}}\right)\\&\quad+\Bigl(- \frac{\left(\zeta - 1\right) \left(\zeta + 1\right) \left(\zeta^{2} + 1\right)}{8 P_{q}^{3} \zeta^{2}}\Bigr)\mathrm{Li}_2\!\left(- \frac{\left(\zeta - 1\right) \left(\zeta + 1\right)}{R \zeta^{2} + 1}\right)\\&\quad+\Bigl(\frac{\left(R + \zeta^{2}\right) \left(R \zeta^{2} - 1\right)}{8 P_{q}^{3} R \zeta^{2}}\Bigr)\mathrm{Li}_2\!\left(\frac{1}{R \zeta^{2} + 1}\right)\\&\quad+\Bigl(\frac{\left(R - 1\right) \left(R + 1\right)}{8 P_{q}^{3} R}\Bigr)\mathrm{Li}_2\!\left(\frac{\zeta^{2} \left(R + 1\right)}{R + \zeta^{2}}\right)\\&\quad+\Bigl(- \frac{\left(R - 1\right) \left(R + 1\right)}{8 P_{q}^{3} R}\Bigr)\mathrm{Li}_2\!\left(\frac{\zeta^{2} \left(R + 1\right)}{R \zeta^{2} + 1}\right)\\&\quad+\Bigl(- \frac{\left(\zeta - 1\right) \left(\zeta + 1\right) \left(\zeta^{2} + 1\right)}{8 P_{q}^{3} \zeta^{2}}\Bigr)\mathrm{Li}_2\!\left(\frac{R \left(\zeta - 1\right) \left(\zeta + 1\right)}{R \zeta^{2} + 1}\right)\\&\quad+\Bigl(\frac{\left(R + \zeta^{2}\right) \left(R \zeta^{2} - 1\right)}{8 P_{q}^{3} R \zeta^{2}}\Bigr)\mathrm{Li}_2\!\left(\frac{R \zeta^{2}}{R \zeta^{2} + 1}\right)\\&\quad+\Bigl(\frac{\left(R - 1\right) \left(R + 1\right)}{8 P_{q}^{3} R}\Bigr)\mathrm{Li}_2\!\left(\frac{R + 1}{R + \zeta^{2}}\right)\\&\quad+\Bigl(- \frac{\left(R - \zeta^{2}\right) \left(R \zeta^{2} + 1\right)}{8 P_{q}^{3} R \zeta^{2}}\Bigr)\mathrm{Li}_2\!\left(\frac{R}{R + \zeta^{2}}\right)\\&\quad+\Bigl(- \frac{\left(R - 1\right) \left(R + 1\right)}{8 P_{q}^{3} R}\Bigr)\mathrm{Li}_2\!\left(\frac{R + 1}{R \zeta^{2} + 1}\right)\\&\quad+\Bigl(\frac{R^{2} + 1}{8 P_{q}^{3} R}\Bigr)\mathrm{Li}_2\!\left(\frac{1}{\zeta^{2}}\right)\\&\quad+\Bigl(- \frac{R^{2} + 1}{8 P_{q}^{3} R}\Bigr)\mathrm{Li}_2\!\left(\zeta^{2}\right)\\&\quad+\Bigl(- \frac{\left(\zeta - 1\right) \left(\zeta + 1\right) \left(\zeta^{2} + 1\right)}{8 P_{q}^{3} \zeta^{2}}\Bigr)\mathrm{Li}_2\!\left(\frac{\left(\zeta - 1\right) \left(\zeta + 1\right)}{R + \zeta^{2}}\right)\\&\quad+\Bigl(- \frac{\left(R - \zeta^{2}\right) \left(R \zeta^{2} + 1\right)}{8 P_{q}^{3} R \zeta^{2}}\Bigr)\mathrm{Li}_2\!\left(\frac{\zeta^{2}}{R + \zeta^{2}}\right)\\&\quad+\Bigl(\frac{1}{4 P_{q}^{3}}\Bigr)S\!\left(\frac{1}{\zeta^{2}},- \frac{1}{R}\right)\\&\quad+\Bigl(\frac{1}{4 P_{q}^{3}}\Bigr)S\!\left(\frac{1}{\zeta^{2}},- R\right)\\&\quad+\Bigl(- \frac{1}{4 P_{q}^{3}}\Bigr)S\!\left(\zeta^{2},- \frac{1}{R}\right)\\&\quad+\Bigl(- \frac{1}{4 P_{q}^{3}}\Bigr)S\!\left(\zeta^{2},- R\right)\\&\quad+\frac{1}{8 P_{q}^{3} R \zeta^{2}}\Bigl[- 2 \zeta^{2} \ell_{\zeta} + 2 R \ell_{\zeta^2-1} + \zeta^{2} \ell_{R} \ell_{1+R\zeta^2} - \zeta^{2} \ell_{R} \ell_{R+\zeta^2}\\&\qquad- 2 R \ell_{R} \ell_{\zeta} - 2 R^{2} \zeta^{2} \ell_{\zeta} - 2 \zeta^{2} \ell_{1+R\zeta^2} \ell_{1+R} - 2 R \ell_{1+R\zeta^2} \ell_{\zeta^2-1}\\&\qquad- 2 R \ell_{R+\zeta^2} \ell_{\zeta^2-1} - 2 R \zeta^{4} \ell_{\zeta^2-1} + 2 R \ell_{R} \ell_{\zeta^2-1} + 2 R \ell_{\zeta} \ell_{1+R\zeta^2}\\&\qquad+2 R \ell_{\zeta} \ell_{R+\zeta^2} + 2 \zeta^{2} \ell_{1+R} \ell_{R+\zeta^2} + 4 R \ell_{\zeta} \ell_{\zeta^2-1} + 4 R \zeta^{4} \ell_{\zeta}\\&\qquad+R^{2} \zeta^{2} \ell_{R} \ell_{R+\zeta^2} - R^{2} \zeta^{2} \ell_{R} \ell_{1+R\zeta^2} - 4 R \zeta^{4} \ell_{\zeta} \ell_{\zeta^2-1} - 2 R \zeta^{4} \ell_{R} \ell_{\zeta^2-1}\\&\qquad- 2 R \zeta^{4} \ell_{\zeta} \ell_{1+R\zeta^2} - 2 R \zeta^{4} \ell_{\zeta} \ell_{R+\zeta^2} - 2 R^{2} \zeta^{2} \ell_{1+R} \ell_{R+\zeta^2} + 2 R \zeta^{4} \ell_{R} \ell_{\zeta}\\&\qquad+2 R^{2} \zeta^{2} \ell_{1+R\zeta^2} \ell_{1+R} + 2 R \zeta^{4} \ell_{1+R\zeta^2} \ell_{\zeta^2-1} + 2 R \zeta^{4} \ell_{R+\zeta^2} \ell_{\zeta^2-1}\Bigr]\end{align*}

\begin{align*}F_c(\zeta,R)&=\Bigl(\frac{\ell_{\zeta}}{P_{q}}\Bigr)\mathrm{Li}_2\!\left(- \frac{1}{R}\right)\\&\quad+\Bigl(\frac{\ell_{\zeta}}{P_{q}}\Bigr)\mathrm{Li}_2\!\left(- R\right)\\&\quad+\Bigl(- \frac{1}{2 P_{q}}\Bigr)S\!\left(\frac{1}{\zeta^{2}},- \frac{1}{R}\right)\\&\quad+\Bigl(- \frac{1}{2 P_{q}}\Bigr)S\!\left(\frac{1}{\zeta^{2}},- R\right)\\&\quad+\Bigl(\frac{1}{2 P_{q}}\Bigr)S\!\left(\zeta^{2},- \frac{1}{R}\right)\\&\quad+\Bigl(\frac{1}{2 P_{q}}\Bigr)S\!\left(\zeta^{2},- R\right)\end{align*}

\begin{align*}F_d(\zeta,R)&=\Bigl(- \frac{2 \left(\zeta - 1\right) \left(\zeta + 1\right)}{P_{q} \left(\zeta^{2} + 1\right)}\Bigr)\mathrm{Li}_2\!\left(- \frac{1}{R - 1}\right)\\&\quad+\Bigl(\frac{2 \left(\zeta - 1\right) \left(\zeta + 1\right)}{P_{q} \left(\zeta^{2} + 1\right)}\Bigr)\mathrm{Li}_2\!\left(- \frac{2}{R - 1}\right)\\&\quad+\Bigl(- \frac{2 \zeta^{2}}{P_{q} \left(\zeta^{2} + 1\right)}\Bigr)\mathrm{Li}_2\!\left(- \frac{R \left(\zeta - 1\right) \left(\zeta + 1\right)}{R + \zeta^{2}}\right)\\&\quad+\Bigl(- \frac{2 \zeta^{2}}{P_{q} \left(\zeta^{2} + 1\right)}\Bigr)\mathrm{Li}_2\!\left(- \frac{\left(\zeta - 1\right) \left(\zeta + 1\right)}{R \zeta^{2} + 1}\right)\\&\quad+\Bigl(- \frac{2 \left(R + \zeta^{2}\right)}{P_{q} \left(R - 1\right) \left(\zeta^{2} + 1\right)}\Bigr)\mathrm{Li}_2\!\left(\frac{1}{R \zeta^{2} + 1}\right)\\&\quad+\Bigl(\frac{2}{P_{q}}\Bigr)\mathrm{Li}_2\!\left(\frac{1}{\zeta^{2} + 1}\right)\\&\quad+\Bigl(\frac{2 \left(\zeta - 1\right) \left(\zeta + 1\right)}{P_{q} \left(\zeta^{2} + 1\right)}\Bigr)\mathrm{Li}_2\!\left(\frac{2 R}{R - 1}\right)\\&\quad+\Bigl(\frac{2}{P_{q}}\Bigr)\mathrm{Li}_2\!\left(\frac{2 \zeta^{2}}{\zeta^{2} + 1}\right)\\&\quad+\Bigl(- \frac{2}{P_{q}}\Bigr)\mathrm{Li}_2\!\left(\frac{2}{\zeta^{2} + 1}\right)\\&\quad+\Bigl(- \frac{2 R}{P_{q} \left(R - 1\right)}\Bigr)\mathrm{Li}_2\!\left(\frac{\zeta^{2} \left(R + 1\right)}{R + \zeta^{2}}\right)\\&\quad+\Bigl(\frac{2}{P_{q} \left(R - 1\right)}\Bigr)\mathrm{Li}_2\!\left(\frac{\zeta^{2} \left(R + 1\right)}{R \zeta^{2} + 1}\right)\\&\quad+\Bigl(\frac{2}{P_{q} \left(\zeta^{2} + 1\right)}\Bigr)\mathrm{Li}_2\!\left(\frac{R \left(\zeta - 1\right) \left(\zeta + 1\right)}{R \zeta^{2} + 1}\right)\\&\quad+\Bigl(- \frac{2 \left(R + \zeta^{2}\right)}{P_{q} \left(R - 1\right) \left(\zeta^{2} + 1\right)}\Bigr)\mathrm{Li}_2\!\left(\frac{R \zeta^{2}}{R \zeta^{2} + 1}\right)\\&\quad+\Bigl(- \frac{2}{P_{q} \left(R - 1\right)}\Bigr)\mathrm{Li}_2\!\left(\frac{R + 1}{R + \zeta^{2}}\right)\\&\quad+\Bigl(\frac{2 \left(R \zeta^{2} + 1\right)}{P_{q} \left(R - 1\right) \left(\zeta^{2} + 1\right)}\Bigr)\mathrm{Li}_2\!\left(\frac{R}{R + \zeta^{2}}\right)\\&\quad+\Bigl(- \frac{2 \left(\zeta - 1\right) \left(\zeta + 1\right)}{P_{q} \left(\zeta^{2} + 1\right)}\Bigr)\mathrm{Li}_2\!\left(\frac{R}{R - 1}\right)\\&\quad+\Bigl(\frac{2 R}{P_{q} \left(R - 1\right)}\Bigr)\mathrm{Li}_2\!\left(\frac{R + 1}{R \zeta^{2} + 1}\right)\\&\quad+\Bigl(\frac{2}{P_{q} \left(\zeta^{2} + 1\right)}\Bigr)\mathrm{Li}_2\!\left(\frac{\left(\zeta - 1\right) \left(\zeta + 1\right)}{R + \zeta^{2}}\right)\\&\quad+\Bigl(\frac{2 \left(R \zeta^{2} + 1\right)}{P_{q} \left(R - 1\right) \left(\zeta^{2} + 1\right)}\Bigr)\mathrm{Li}_2\!\left(\frac{\zeta^{2}}{R + \zeta^{2}}\right)\\&\quad+\Bigl(- \frac{2}{P_{q}}\Bigr)\mathrm{Li}_2\!\left(\frac{\zeta^{2}}{\zeta^{2} + 1}\right)\\&\quad+\frac{1}{P_{q} \left(R - 1\right) \left(\zeta^{2} + 1\right)}\Bigl[- 4 \ell_{\zeta} \ell_{1+R\zeta^2} - 4 \ell_{\zeta} \ell_{R+\zeta^2} - 4 \ell_{1-R} \log{\left(2 \right)} - 2 g_{R} \log{\left(2 \right)}\\&\qquad- 2 h_{R} \ell_{\zeta^2-1} - 2 \ell_{R} \ell_{R+\zeta^2} - 2 \ell_{R} \ell_{\zeta^2-1} - 2 \ell_{1+R\zeta^2} \ell_{1+R}\\&\qquad+2 g_{R} \ell_{\zeta^2-1} + 2 h_{R} \log{\left(2 \right)} + 2 \ell_{R} \ell_{1+R\zeta^2} + 2 \ell_{R} \log{\left(2 \right)}\\&\qquad+2 \ell_{1+R\zeta^2} \ell_{\zeta^2-1} + 2 \ell_{1+R} \ell_{R+\zeta^2} + 2 \ell_{R+\zeta^2} \ell_{\zeta^2-1} + 4 \ell_{R} \ell_{\zeta}\\&\qquad- 4 \zeta^{2} h_{R} \ell_{\zeta} - 4 R \ell_{R} \ell_{\zeta} - 2 R g_{R} \ell_{\zeta^2-1} - 2 \zeta^{2} g_{R} \ell_{\zeta^2-1}\\&\qquad- 2 R h_{R} \log{\left(2 \right)} - 2 \zeta^{2} h_{R} \log{\left(2 \right)} - 2 \zeta^{2} \ell_{R} \ell_{R+\zeta^2} - 2 R \ell_{R} \log{\left(2 \right)}\\&\qquad- 2 \zeta^{2} \ell_{R} \log{\left(2 \right)} - 2 R \ell_{1+R\zeta^2} \ell_{1+R} - 2 \zeta^{2} \ell_{1+R\zeta^2} \ell_{1+R} - 2 R \ell_{1+R\zeta^2} \ell_{\zeta^2-1}\\&\qquad- 2 \zeta^{2} \ell_{1+R\zeta^2} \ell_{\zeta^2-1} - 2 R \ell_{R+\zeta^2} \ell_{\zeta^2-1} - 2 \zeta^{2} \ell_{R+\zeta^2} \ell_{\zeta^2-1} + 2 R g_{R} \log{\left(2 \right)}\\&\qquad+2 \zeta^{2} g_{R} \log{\left(2 \right)} + 2 R h_{R} \ell_{\zeta^2-1} + 2 \zeta^{2} h_{R} \ell_{\zeta^2-1} + 2 \zeta^{2} \ell_{R} \ell_{1+R\zeta^2}\\&\qquad+2 R \ell_{R} \ell_{\zeta^2-1} + 2 \zeta^{2} \ell_{R} \ell_{\zeta^2-1} + 2 R \ell_{1+R} \ell_{R+\zeta^2} + 2 \zeta^{2} \ell_{1+R} \ell_{R+\zeta^2}\\&\qquad+4 \zeta^{2} g_{R} \ell_{\zeta} + 4 R \ell_{\zeta} \ell_{1+R\zeta^2} + 4 R \ell_{\zeta} \ell_{R+\zeta^2} + 4 R \ell_{1-R} \log{\left(2 \right)}\\&\qquad+4 \zeta^{2} \ell_{1-R} \log{\left(2 \right)} + 8 \zeta^{2} \ell_{\zeta} \ell_{\zeta^2-1} - 8 R \zeta^{2} \ell_{\zeta} \ell_{\zeta^2-1} - 4 R \zeta^{2} g_{R} \ell_{\zeta}\\&\qquad- 4 R \zeta^{2} \ell_{1-R} \log{\left(2 \right)} - 2 R \zeta^{2} g_{R} \log{\left(2 \right)} - 2 R \zeta^{2} h_{R} \ell_{\zeta^2-1} - 2 R \zeta^{2} \ell_{R} \ell_{\zeta^2-1}\\&\qquad- 2 R \zeta^{2} \ell_{1+R\zeta^2} \ell_{1+R} + 2 R \zeta^{2} g_{R} \ell_{\zeta^2-1} + 2 R \zeta^{2} h_{R} \log{\left(2 \right)} + 2 R \zeta^{2} \ell_{R} \log{\left(2 \right)}\\&\qquad+2 R \zeta^{2} \ell_{1+R\zeta^2} \ell_{\zeta^2-1} + 2 R \zeta^{2} \ell_{1+R} \ell_{R+\zeta^2} + 2 R \zeta^{2} \ell_{R+\zeta^2} \ell_{\zeta^2-1} + 4 R \zeta^{2} h_{R} \ell_{\zeta}\Bigr]\end{align*}

